Vertical shear instability in two-moment radiation-hydrodynamical simulations of irradiated protoplanetary disks II. Secondary instabilities and stability regions

The vertical shear instability (VSI) is a hydrodynamical instability likely to produce turbulence in the dead zones of protoplanetary disks. Various aspects of this instability remain to be understood, including the disk regions where it can operate and the physical phenomena leading to its saturation. In this work, we studied the growth and evolution of secondary instabilities parasitic to the VSI, examining their relation with its saturation in axisymmetric radiation-hydrodynamical simulations of protoplanetary disks. We also constructed stability maps for our disk models, considering temperature stratifications enforced by stellar irradiation and radiative cooling and incorporating the effects of dust-gas collisions and molecular line emission. We found that the flow pattern produced by the interplay of the axisymmetric VSI modes and the baroclinic torque forms bands of nearly uniform specific angular momentum. In the high-shear regions in between these bands, the Kelvin-Helmholtz instability (KHI) is triggered. The significant transfer of kinetic energy to small-scale eddies produced by the KHI and possibly even the baroclinic acceleration of eddies limit the maximum energy of the VSI modes, likely leading to the saturation of the VSI. A third instability mechanism, consisting of an amplification of eddies by baroclinic torques, forms meridional vortices with Mach numbers up to $\sim 0.4$. Our stability analysis suggests that protoplanetary disks can be VSI-unstable in surface layers up to tens of au for reasonably high gas emissivities, even in regions where the midplane is stable. This picture is consistent with current observations of disks showing thin midplane millimeter-sized dust layers while appearing vertically extended in optical and near-infrared wavelengths.

==> diskmodel.tex <==
 \section{Disk structure and stability}\label{S:DiskModel}
 
 \subsection{Initial condition} \label{S:InitialCondition}
 
The hydrostatic equilibrium conditions can
be obtained by setting all time derivatives to zero in Eqs. \eqref{Eq:RadHD}.
Additionally, we neglect viscous and radiative momentum exchange by setting $\mathbf{G}$ to zero. This
choice is justified since... \GREEN(order of magnitude)\BLACK
Thus, the $(r,\theta)$ components of the static momentum conservation equation are
\begin{equation}\label{Eq:Hydrostatic}
    \begin{split}
        \frac{\partial p_g}{\partial r} &=
        -\rho \frac{\partial \Phi}{\partial r}
        + \frac{\rho v_\phi^2}{r}  \\
        \frac{1}{r} \frac{\partial p_g}{\partial \theta}
        & = \frac{1}{\tan \theta}  \frac{\rho v_\phi^2}{r}\,.
    \end{split}
\end{equation}
The equilibrium configuration is obtained by
assuming a given vertically integrated density
distribution $\Sigma(r)$. The midplane gas
density is then computed in
terms of the local scale heigth
$H=\sqrt{(\mu u T_m/k_B)\, r^3/G M_s}$ as
$\rho(r,\theta=\pi/2)=\Sigma (r)/\sqrt{2\pi}H$, where $M_s$ is the star mass and $T_m$ is the
midplane temperature. This approximation holds
if the mass distribution is vertically Gaussian, which is true close to the midplane provided the temperature profile is vertically isothermal. 
This condition is in fact ferified close to 
the midplane, where most of the mass is located.
Once the midplane density is known, Eq.
\eqref{Eq:Hydrostatic} is integrated as detailed
in \cite{Flock2013} using the known temperature
distribution, and new $(\rho,v_\phi)$ values
are computed in the entire domain. The
Rad-HD equations are then integrated assuming the new configuration to be static \GREEN(rewrite)\BLACK,
and a new temperature distribution  is obtained. The whole process is repeated until convergence
of the temperature and density distributions \GREEN(convergence criterion)\BLACK.

\GREEN Boundary conds.  \BLACK

